PlayVirtual: Augmenting Cycle-Consistent Virtual Trajectories for Reinforcement Learning

Learning good feature representations is important for deep reinforcement learning (RL). However, with limited experience, RL often suffers from data inefficiency for training. For un-experienced or less-experienced trajectories (i.e., state-action sequences), the lack of data limits the use of them for better feature learning. In this work, we propose a novel method, dubbed PlayVirtual, which augments cycle-consistent virtual trajectories to enhance the data efficiency for RL feature representation learning. Specifically, PlayVirtual predicts future states in the latent space based on the current state and action by a dynamics model and then predicts the previous states by a backward dynamics model, which forms a trajectory cycle. Based on this, we augment the actions to generate a large amount of virtual state-action trajectories. Being free of groudtruth state supervision, we enforce a trajectory to meet the cycle consistency constraint, which can significantly enhance the data efficiency. We validate the effectiveness of our designs on the Atari and DeepMind Control Suite benchmarks. Our method achieves the state-of-the-art performance on both benchmarks.

==> tables/ablation_Aug.tex <==
% \begin{wraptable}{r}{7.cm}
\begin{table*}[h]
    % \footnotesize % control font size
    % \scriptsize
    \centering
    \caption{Exploring the effectiveness of our virtual trajectory augmentation. We report median HNS ($\%$) on Atari-100k and median score on DMControl-100k and DMControl-500k.}
    \label{table:ablation_loss}
    % \vskip 0.05in    % control the gap between caption and table
    % \setlength{\tabcolsep}{2.0mm}{
    % \resizebox{\textwidth}{!}{
    \scalebox{0.88}{
        \begin{tabular}{l c c c c c c}
            \toprule
            \textbf{Model} & Pred & Rec & AugVir & $\textbf{Atari-100k}$ & $\textbf{DMC-100k}$ & $\textbf{DMC-500k}$\\
            % \midrule
            % Distance Based Models
            \midrule
            SPR\bmark           & \checkmark    & & & &  &  \\
            SPR\bmark+Rec    & \checkmark     & \checkmark  & & & &  \\
            SPR\bmark+Vir (Ours)    & \checkmark &    & \checkmark & &  &  \\
            SPR\bmark+Rec+Vir   & \checkmark    &  \checkmark &  \checkmark & &  & \\
            \bottomrule
        \end{tabular}
    }
    % \vspace{0pt}   % control the gap between the table bottom and next paragraph
% \end{wraptable}
\end{table*}



% % \begin{wraptable}{r}{7.cm}
% \begin{table*}[h]
%     % \footnotesize % control font size
%     % \scriptsize
%     \centering
%     \caption{Ablation of RDM supervision.}
%     \label{table:ablation_loss}
%     % \vskip 0.05in    % control the gap between caption and table
%     % \setlength{\tabcolsep}{2.0mm}{
%     % \resizebox{\textwidth}{!}{
%     \scalebox{0.88}{
%         \begin{tabular}{l c c c c c c}
%             \toprule
%             \textbf{Model} & Cycle & Rec & Rec() & $\textbf{Atari-100k}$ & $\textbf{DMC-100k}$ & $\textbf{DMC-500k}$\\
%             % \midrule
%             % Distance Based Models
%             \midrule
%             Option 1 (Ours)           & \checkmark    & & & &  &  \\
%             Option 2    & \checkmark     & \checkmark  & & & &  \\
%             Option 3    & \checkmark    &  &  \checkmark & &  & \\
%             \bottomrule
%         \end{tabular}
%     }
%     % \vspace{0pt}   % control the gap between the table bottom and next paragraph
% % \end{wraptable}
% \end{table*}


==> tables/ablation_DM_BDM.tex <==
% \begin{table}[H]
% \begin{minipage}{0.48\linewidth}
% % \centering
% % \vspace{-2pt}
% \centering
% \caption{Exploring the effect of the proposed cycle scheme on DM.}
% % \caption{Exploring the effect of the proposed cycle scheme on DM. \ourname-NG is the \ourname~ without the cycle loss updating on DM.}
%     \scalebox{0.8}{
%         \begin{tabular}{l l c }
%             \toprule
%             % &\textbf{K} & \textbf{0} & \textbf{3} & \textbf{6} & \textbf{9} & \textbf{12} \\
%             \textbf{Benchmark} & \textbf{Model} & \textbf{Performance} \\
%             \midrule
%             \multirow{3}{*}{Atari-100k}  & SPR & 37.1 \\
%             & \ourname-NG & 44.0 \\
%             & \ourname & \textbf{47.2} \\
%             \midrule
%             \multirow{3}{*}{DMC-100k}  & SPR\bmark & 728.0 \\
%             & \ourname-NG & 777.5 \\
%             & \ourname & \textbf{797.0} \\
%             \bottomrule
%         \end{tabular}
%     }
% \end{minipage}
% \vspace{-2pt}
% \hspace{5mm}
% \begin{minipage}{0.48\linewidth}  
% \centering
% \caption{Ablation of adding extra groundtruth supervision to BDM on DMControl-100k.}
%         \begin{tabular}{l c}
%             \toprule
%             \textbf{Model} & $\textbf{Median Score}$\\
%             % \midrule
%             % Distance Based Models
%             \midrule
%             SPR\bmark       &  723.0 \\
%             SPR\bmark+BDM & 720.0 \\
%             SPR\bmark+BDM+Cycle & 771.0 \\
%             SPR\bmark+Cycle (Ours) & 797.0 \\
%             \bottomrule
%         \end{tabular} \label{table:ablation_BDM}
% \end{minipage}
% \vspace{-2pt}
% \end{table}



\begin{table}[H]
\begin{minipage}{0.48\linewidth}
\centering
\caption{Ablation of adding extra groundtruth supervision to BDM on DMControl-100k.}
        \begin{tabular}{l c}
            \toprule
            \textbf{Model} & $\textbf{Median Score}$\\
            % \midrule
            % Distance Based Models
            \midrule
            SPR\bmark       &  723.0 \\
            SPR\bmark+BDM   &  \\
            SPR\bmark+BDM+Cycle &  \\
            SPR\bmark+Cycle (Ours) & 797.0 \\
            \bottomrule
        \end{tabular} \label{table:ablation_BDM}
\end{minipage}
\vspace{-2pt}
\hspace{5mm}
\begin{minipage}{0.48\linewidth}  
% \centering
% \vspace{-2pt}
\centering
\caption{Exploring the effect of the proposed cycle scheme on DM. \ourname-NG is the \ourname~ without the cycle loss updating on DM.}
        \begin{tabular}{l c c}
            \toprule
            \textbf{Model} & $\textbf{Atari-100k}$ & $\textbf{DMC-100k}$ \\
            % \midrule
            % Distance Based Models
            \midrule
            Baseline       &  37.1 & 723.0 \\
            \ourname-NG & 44.0  & 777.5 \\
            \ourname & 47.2 & 797.0 \\
            \bottomrule
        \end{tabular} \label{table:ablation_DM}
\end{minipage}
\vspace{-2pt}
\end{table}

==> tables/ablation_option.tex <==
% \begin{wraptable}{r}{7.cm}
\begin{table*}[h]
% \vspace{-4mm}
    % \footnotesize % control font size
    % \scriptsize
    \centering
    %the strong baseline
    \caption{Exploring the options of our cycle scheme including metric space, the location of applying cycle consistency constraint and warmup scheme.}
    %Comparing models with different losses. We report median HNS ($\%$) on Atari-100k and the median score on DMControl-100k and DMControl-500k. 
    \label{table:ablation_option}
    % \vskip 0.05in    % control the gap between caption and table
    % \setlength{\tabcolsep}{2.0mm}{
    % \resizebox{\textwidth}{!}{
    \scalebox{1.0}{
        \begin{tabular}{c c c c c c }
            \toprule
            \textbf{Metric Space} & \textbf{Contraint Location} & \textbf{Warmup} & $\textbf{Atari-100k}$ & $\textbf{DMControl-100k}$\\
            % \midrule
            % Distance Based Models
            \midrule
            feature & end step & yes & 44.8 & 798.5 \\
            projection & every step & yes & 46.1 & 781.0 \\
            projection & end step & no & 42.5 & 749.5 \\
            projection & end step & yes & 47.2 & 797.0 \\
            \bottomrule
        \end{tabular}
    }
    % \vspace{-6pt}   % control the gap between the table bottom and next paragraph
% \end{wraptable}
\end{table*}



% % \begin{wraptable}{r}{7.cm}
% \begin{table*}[h]
% % \vspace{-4mm}
%     % \footnotesize % control font size
%     % \scriptsize
%     \centering
%     %the strong baseline
%     \caption{Exploring the influence of metric space, the location of applying cycle consistency constraint and warmup scheme.}
%     %Comparing models with different losses. We report median HNS ($\%$) on Atari-100k and the median score on DMControl-100k and DMControl-500k. 
%     \label{table:ablation_metric}
%     % \vskip 0.05in    % control the gap between caption and table
%     % \setlength{\tabcolsep}{2.0mm}{
%     % \resizebox{\textwidth}{!}{
%     \scalebox{0.85}{
%         \begin{tabular}{c c c c c c c c}
%             \toprule
%             \multicolumn{2}{c}{\textbf{Metric Space}} & \multicolumn{2}{c}{\textbf{Contraint Location}} & \multicolumn{2}{c}{\textbf{Warmup}} & $\textbf{Atari-100k}$ & $\textbf{DMControl-100k}$\\
%             % \midrule
%             % Distance Based Models
%             \midrule
%             % feature &  &   \\
%             % projection & 47.2 & 797.0 \\
%             \bottomrule
%         \end{tabular}
%     }
%     % \vspace{-6pt}   % control the gap between the table bottom and next paragraph
% % \end{wraptable}
% \end{table*}



% % \begin{wraptable}{r}{7.cm}
% \begin{table*}[h]
% % \vspace{-4mm}
%     % \footnotesize % control font size
%     % \scriptsize
%     \centering
%     %the strong baseline
%     \caption{Exploring the influence of metric space.}
%     %Comparing models with different losses. We report median HNS ($\%$) on Atari-100k and the median score on DMControl-100k and DMControl-500k. 
%     \label{table:ablation_metric}
%     % \vskip 0.05in    % control the gap between caption and table
%     % \setlength{\tabcolsep}{2.0mm}{
%     % \resizebox{\textwidth}{!}{
%     \scalebox{0.85}{
%         \begin{tabular}{l c c }
%             \toprule
%             \textbf{Metric Space} & $\textbf{Atari-100k}$ & $\textbf{DMControl-100k}$\\
%             % \midrule
%             % Distance Based Models
%             \midrule
%             % Baseline      & N/A & 37.1 & 728.0 \\
%             feature &  &   \\
%             projection & 47.2 & 797.0 \\
%             \bottomrule
%         \end{tabular}
%     }
%     % \vspace{-6pt}   % control the gap between the table bottom and next paragraph
% % \end{wraptable}
% \end{table*}





% % \begin{wraptable}{r}{7.cm}
% \begin{table*}[h]
% % \vspace{-4mm}
%     % \footnotesize % control font size
%     % \scriptsize
%     \centering
%     %the strong baseline
%     \caption{Exploring the influence of metric space.}
%     %Comparing models with different losses. We report median HNS ($\%$) on Atari-100k and the median score on DMControl-100k and DMControl-500k. 
%     \label{table:ablation_metric}
%     % \vskip 0.05in    % control the gap between caption and table
%     % \setlength{\tabcolsep}{2.0mm}{
%     % \resizebox{\textwidth}{!}{
%     \scalebox{0.85}{
%         \begin{tabular}{l c c c }
%             \toprule
%             \textbf{Model} & \textbf{Metric Space} & $\textbf{Atari-100k}$ & $\textbf{DMControl-100k}$\\
%             % \midrule
%             % Distance Based Models
%             \midrule
%             % Baseline      & N/A & 37.1 & 728.0 \\
%             \multirow{2}{*}{\ourname}     & feature &  &   \\
%                   & projection& 47.2 & 797.0 \\
%             \bottomrule
%         \end{tabular}
%     }
%     % \vspace{-6pt}   % control the gap between the table bottom and next paragraph
% % \end{wraptable}
% \end{table*}

==> tables/dynamics.tex <==
% % \begin{wraptable}{r}{7.cm}
% \begin{table*}[h]
%     % \footnotesize % control font size
%     % \scriptsize
%     \centering
%     \caption{Comparison of three kinds of dynamics.}
%     \label{table:dynamics}
%     % \vskip 0.05in    % control the gap between caption and table
%     % \setlength{\tabcolsep}{2.0mm}{
%     % \resizebox{\textwidth}{!}{
%     \scalebox{0.88}{
%         \begin{tabular}{l c c c c c c c c c c}
%             \toprule
%             \textbf{Function} & \textbf{Space} & \textbf{Definition}\\
%             % \midrule
%             % Distance Based Models
%             \midrule
%             Dynamics           & $\mathcal{S}\times \mathcal{A}\rightarrow \mathcal{S}$     & 
%             $ Pr(s_{t+1}|s_t, a_t)$\\
%             Inverse dynamics   & $\mathcal{S}\times \mathcal{S}\rightarrow \mathcal{A}$     & 
%             $ Pr(a_t|s_t, s_{t+1})$ \\
%             Reverse dynamics   & $\mathcal{S}\times \mathcal{A}\rightarrow \mathcal{S}$     & 
%             $ Pr(s_t|s_{t+1}, a_t)$  \\
%             \bottomrule
%         \end{tabular}
%     }
%     % \vspace{0pt}   % control the gap between the table bottom and next paragraph
% % \end{wraptable}
% \end{table*}


\begin{wraptable}{r}{7.cm}
    % \footnotesize % control font size
    % \scriptsize
    \centering
    \caption{Comparison of three kinds of dynamics.}
    \label{table:dynamics}
    % \vskip 0.05in    % control the gap between caption and table
    % \setlength{\tabcolsep}{2.0mm}{
    % \resizebox{\textwidth}{!}{
    \scalebox{0.88}{
        \begin{tabular}{l c c c c c c c c c c}
            \toprule
            \textbf{Function} & \textbf{Space} & \textbf{Definition}\\
            % \midrule
            % Distance Based Models
            \midrule
            Dynamics           & $\mathcal{S}\times \mathcal{A}\rightarrow \mathcal{S}$     & 
            $ Pr(s_{t+1}|s_t, a_t)$\\
            Inverse dynamics   & $\mathcal{S}\times \mathcal{S}\rightarrow \mathcal{A}$     & 
            $ Pr(a_t|s_t, s_{t+1})$ \\
            Backward dynamics   & $\mathcal{S}\times \mathcal{A}\rightarrow \mathcal{S}$     & 
            $ Pr(s_t|s_{t+1}, a_t)$  \\
            \bottomrule
        \end{tabular}
    }
    % \vspace{0pt}   % control the gap between the table bottom and next paragraph
\end{wraptable}
